Sample Efficient Myopic Exploration Through Multitask Reinforcement Learning with Diverse Tasks

Multitask Reinforcement Learning (MTRL) approaches have gained increasing attention for its wide applications in many important Reinforcement Learning (RL) tasks. However, while recent advancements in MTRL theory have focused on the improved statistical efficiency by assuming a shared structure across tasks, exploration--a crucial aspect of RL--has been largely overlooked. This paper addresses this gap by showing that when an agent is trained on a sufficiently diverse set of tasks, a generic policy-sharing algorithm with myopic exploration design like $\epsilon$-greedy that are inefficient in general can be sample-efficient for MTRL. To the best of our knowledge, this is the first theoretical demonstration of the "exploration benefits" of MTRL. It may also shed light on the enigmatic success of the wide applications of myopic exploration in practice. To validate the role of diversity, we conduct experiments on synthetic robotic control environments, where the diverse task set aligns with the task selection by automatic curriculum learning, which is empirically shown to improve sample-efficiency.

==> Submission/Sec1_Introduction.tex <==
\section{Introduction}

The theory and practice of Reinforcement Learning (RL) differ significantly when it comes to the design of exploration strategies. Many algorithms with carefully designed exploration have been shown sample-efficient with near-optimal regret guarantees or sample complexity guarantees. Popular exploration designs includes Optimism in Face of Uncertainty \cite{auer2008near,bartlett2009regal,dann2017unifying}, Posterior Sampling \citep{osband2017posterior} and random exploration  \cite{xiong2021randomized,xu2019worst}, which often perturbs an empirical estimate of the unknown environment. Nevertheless, these exploration strategies heavily rely on the strong structural assumptions on the underlying environments, which often leads to intractable or non-robust algorithms in practice. Recent work \cite{zhang2021made} has adapted empirical versions of Upper Confidence Bound (UCB), which is shown to improve their efficiency. In practical settings, curiosity-driven exploration has been applied in many real-world applications \citep{zhelo2018curiosity}. These exploration strategies are sample efficient because they encourage exploration towards the direction with higher uncertainty. See \cite{amin2021survey} for a more comprehensive survey.

Despite the significant body of literature on exploration strategies, most of the existing empirical works apply myopic exploration, such as $\epsilon$-greedy and entropy-based exploration. Myopic exploration is widely recognized to be sample-inefficient \citep{o2018uncertainty} due to its lack of {\em directed} exploration, which leads to sample complexity exponentially large in the horizon. Nonetheless, RL with myopic exploration has achieved astonishing success in many application domains including Atari game \citep{espeholt2018impala,oh2015action}, robotic control and healthcare \citep{nahum2018just,shin2022modeling}, which poses a mystery as to \textit{why myopic exploration is sample-efficient in practice}.

%\ziping{Mention curiosity. Rmax. They are more intuitive. Cite some survey papers.}

In this paper, we address the problem from the perspective of multitask learned RL. Multitask Learning (MTL) appears to be a fundamental aspect of RL training and many important RL applications can be considered as multitask learning problems. For example, multi-agent deep RL is trained for different Atari games with shared parameters \citep{terry2020revisiting}. Robotic control agents are trained to solve different goals simultaneously in multiple goal-conditioned environments \citep{andreas2017modular,andrychowicz2017hindsight}. Nevertheless, previous theories on Multitask RL (MTRL) have mainly focused on analyzing the shared structure across different tasks, which allows for shared parameters or representation function \citep{agarwal2022provable,lu2021power,cheng2022provable}. This approach is analogous to the benefits of Multitask Supervised Learning and has been well-understood in the literature \citep{du2020few,maurer2016benefit} and these algorithms still rely on carefully designed exploration strategies.  % For instance, \cite{agarwal2022provable} assumes linear MDP \cite{jin2020provably}, where the feature extractor is shared by all the tasks. This approach is analogous to the benefits of Multitask Supervised Learning, which has been well-understood in the literature \citep{maurer2016benefit,du2020few}. 

% By contrast, we propose a new perspective that learning an RL agent for a diverse set of tasks mitigates the difficulty of exploration design, which may allow efficient myopic exploration. We argue that multitask RL is implicitly learning through a curriculum, and the task set is rich enough such that we only need to make one-step exploration to change the optimal policy of one MDP to that of its successor. Therefore, we can leverage the diversity of tasks to facilitate efficient exploration. An illustration of this concept can be found in the RiverSwim example in Figure \ref{fig:illus}.
% Let $T$ be the total number of tasks. This line of work seeks a reduction of $1/\sqrt{T}$ on the complexity of the part shared across tasks.

By contrast, we introduce a new perspective that \textit{learning an RL agent for a \textbf{diverse} set of tasks mitigates the difficulty of exploration design, which may allow efficient myopic exploration.} Intuitively, we argue that multitask RL is implicitly learning through a curriculum \ambuj{we mention an implicit curriculum in the intro and in the conclusion. there's a bit of discussion in sec. 3.1 but can sth more concrete be said? none of the results themselve have any curriculum in it so the curriculum in implicit in the analysis?}, and the task set is adequately rich such that we only need to make one step exploration to change the optimal policy of one MDP to that of its
successor. In this way, we can leverage the diversity of tasks to facilitate efficient exploration. %An illustration of this concept can be found in the RiverSwim example in Figure \ref{fig:illus}.

\paragraph{Contributions.} In this paper, we discuss a sufficient diversity condition for achieving sample efficient myopic exploration under a general value function approximation setting \citep{dann2022guarantees,jin2021bellman}. We provide analysis of how a diverse task set satisfies the condition in different cases, including tabular cases, linear cases and linear quadratic regulator cases. In the end, we validate our theory with experiments on real robotic control environments, where we will see that a more plausible task set leads to a better policy learning and an improved generalization performance. 

\subsection{Related Work}

\paragraph{Multitask RL.} A recent line of work tries to understand the benefits of multitask RL with the shared structures \citep{agarwal2022provable,brunskill2013sample,calandriello2014sparse,cheng2022provable, lu2021power,uehara2021representation,yang2022nearly,zhang2021provably}. %\ambuj{only 3? seems like a small number. there must be more papers on MTRL even if we restrict to those w/ theoretical guarantees} 
Studying the benefits of MTL with share structures started from the similar setups in Supervised Learning. This line of works show that learning multiple tasks with a shared structure reduces the generalization error by a factor of $1/\sqrt{T}$. Recently similar settings
are analyzed for MDPs.
In contrast, our work does not focus on the improved statistical efficiency through a shared structure. Instead, we try to understand how a diverse set of tasks implicitly encourages exploration. 
%\cite{lu2021power} showed a similar bound on the sub-optimality of the learned policy for linear MDPs \citep{jin2020provably} under the assumption that least-square value iteration weight matrix from source is full rank. \cite{agarwal2022provable} makes a different assumption that the target transition probability is a linear combination of the source ones, and the feature extractor is shared by all the tasks. 

\paragraph{Myopic exploration.} Myopic exploration is the most commonly used design of exploration as it is easy to implement and it works well in a range of problems, including many of practical interests \citep{kalashnikov2018scalable,mnih2015human}. Many works \citep{dabney2020temporally,dann2022guarantees,liu2018simple,simchowitz2020naive} have discussed the conditions, under which myopic exploration is efficient. All of them consider a single MDP and they require strong conditions on the underlying environment.

\paragraph{Curriculum learning.} Curriculum learning refers to adaptively selecting tasks in a certain order to improve the learning performance \citep{bengio2009curriculum}. There is a enormous amount of literature showing the improved performances in different applications \citep{jiang2015self,pentina2015curriculum,graves2017automated,wang2021survey}. However, there is little theoretical understanding of it. \cite{xu2022statistical} studied the statistical benefits of curriculum learning under Supervised Learning setting. For RL, \cite{li2022understanding} made a first step towards the understanding of sample complexity gains of curriculum learning without an explicit exploration bonus. Their results are under strong assumptions, e.g. prior knowledge on the curriculum and a special contextual RL setting, which assumes Lipschitz rewards. This work can be seen as a more comprehensive framework of such benefits, where we discuss general MDPs with function approximation. We argue that MTRL with myopic exploration is implicitly learning through a curriculum learning.

%\paragraph{Contributions.} We summarize the main contributions of this work in the following aspects.

==> Submission/Sec5_Auto_Task_Scheduler.tex <==
% \section{Automatic Task Scheduler}

% In the previous section, we have discussed Algorithm \ref{alg:generic}, which runs the estimated optimal policies on each MDP once per round. This protocol can be inefficient when we have a large task set and they are heavily biased (a majority of the tasks are identical). In practice, we can have an infinite set of MDPs. Thus, we need a task scheduler that adaptively schedule tasks for learning.

% This can also be beneficial as we discussed that a curriculum be reduce the learning complexity.

% \ziping{Review the literature on automatic curriculum learning.}

% \ziping{Put R-max result here. This is a case, where task set is large and we have to schedule the appropriate MDP at each round. If we have the prior information, we can do R-max type of selection. If we don't, then we have to adaptively select tasks.}

==> Submission/Sec5_Exp_short.tex <==
\vspace{-3mm}

\section{Implications of Diversity in Deep RL}
Though this is a paper focusing on the theoretical justification, we add some preliminary discussion on what diversity means in Deep RL. Thus far, we have provided concrete example for diverse task set in tabular and linear MDPs with lower bounded Multitask MEG. It is often the case that in Deep RL, a pretrained feature extractor is used to generate embeddings for Q-value function and then a linear mapping is applied to generate the final output \citep{bhateja2023robotic,hejna2023few}. This manner is similar to the setup in linear MDPs. We have shown that to achieve diversity for linear MDPs, one important property is to have a full rank covariance matrix of the embeddings at each step $h$ if the optimal policy is executed (Lemma \ref{lem:linear_2}). In this section, we conduct simple simulation studies on BipedalWalker \citep{portelas2020teacher}, a robotic control environment, to verify that whether a more spread spectrum of the covariance matrix of the embeddings would lead to better sample efficiency. 

We found in the experiments that {\it the subset of tasks that leads to more spread spectrum is similar to the task selection of automatic curriculum learning, which has been empirically shown to learn more sample efficiently.} Due to the page limit we provide a high-level summary of the simulation study and the readers can find full details in Appendix \ref{app:experiment_full_details}.

{\bf Experiment setup.} The learning agent is embodied into a bipedal walker whose motors are controlled by continuous actions of torques. The objective of the agent is to move forward as far as possible, while crossing stumps with varying heights at regular intervals. An environment or task, denoted as $M_{p,q}$, is controlled by a parameter vector $(p, q)$, where $p$ and $q$ denote the heights of the stumps and the spacings between the stumps, respectively. % The value $p$ represents the mean of a normal distribution $\mathcal{N}(p, 0.1)$, from which the heights of the stumps are sampled, and the value $q$ determines the spacing between the stumps. 
Intuitively, challenging environments have higher and denser stumps. %We set the parameter ranges for $p$ and $q$ as $p \in [0, 3]$ and $q \in [0, 6]$ in this study. 
The agent is trained by Proximal Policy Optimization (PPO) \citep{schulman2017proximal} with a standard actor-critic framework \citep{konda1999actor} and with Boltzmann exploration that regularizes entropy.
%\footnote{Note that Boltzmann exploration strategy is another example of myopic exploration, which is commonly used for continuous action space. Though it deviates from the $\epsilon$-greedy strategy discussed in the theoretical framework, we remark that the theoretical guarantee outlined in this paper can be trivially extend to Boltzmann exploration.}.
Detailed training setup can be found in Appendix \ref{app:experiment_full_details}.
%The architecture for the actor and critic feature extractors consists of two layers with 400 and 300 neurons, respectively, and Tanh \citep{rumelhart1986learning} as the activation function. Fully-connected layers are then used to compute the action and value. We keep the hyper-parameters for training the agent the same as \citet{romac2021teachmyagent}.

{\bf Proper level of heights leads to more spread spectrum.} 
We evaluate the extracted feature at the end of the training generated by near-optimal policies on 100 tasks with different parameter vectors $(p, q)$. We then compute the covariance matrix of the features for each task, whose spectrum are shown in Figure \ref{fig:cov_mat} (a). We observe that the eigenvalues can be 10 times higher for environments with an appropriate height (1.0-2.3), compared to extremely high and low heights, while they are roughly the same at different levels of spacings. This indicates that choosing an appropriate height is the key to properly scheduling tasks. 

{\bf Coincidence with automatic curriculum learning.} In fact, the task selection is similar to the tasks selected by the state-of-the-art Automatic Curriculum Learning (ACL). We investigate the curricula generated by ALP-GMM \citep{portelas2020teacher}, a well-established curriculum learning algorithm, for training an agent in the BipedalWalker environment for 20 million timesteps. Figure \ref{fig:cov_mat} (b) gives the density plots of the ACL task sampler during the training process, which shows a significant preference over heights in the middle range, with little preference over spacing. Since ACL has been shown to significantly improve the learning performance in BipedalWalker, this is a strong evidence that the diversity notation discussed in this paper truly leads to a better sample complexity even when Deep RL is employed.
\vspace{-10pt}
\begin{figure}[h]
    \centering
    % \begin{subfigure}[b]{0.48\textwidth}
    % \centering
    % \includegraphics[width = 0.8\textwidth]{Figure/env.jpg}
    % \caption{BipedalWalker environment}
    % \end{subfigure}
    %\begin{subfigure}[b]{0.48\textwidth}
    %\includegraphics[width = 0.8\textwidth]{Figure/Bipedal/Heights_boxplot.pdf}
    %\caption{Controlling heights}
    %\end{subfigure}
    % \begin{subfigure}[b]{0.33\textwidth}
    % \includegraphics[width = 1\textwidth]{Figure/Bipedal/heights_zoom_in.pdf}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\textwidth}
    % \includegraphics[width = 1\textwidth]{Figure/Bipedal/Spacing_boxplot.pdf}
    % \caption{Controlling spacings}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.48\textwidth}
    % \includegraphics[width = 1\textwidth]{Figure/Bipedal/heights_zoom_in.pdf}
    % \caption{Controlling heights in the original scale}
    % \end{subfigure}
    %\begin{subfigure}[b]{0.48\textwidth}
    %\centering
    %\includegraphics[width = 0.384\textwidth, height = 0.384\textwidth]{Figure/Bipedal/scatter_20_square.png}
    %\includegraphics[width = 0.384\textwidth, height = 0.384\textwidth]{Figure/Bipedal/scatter_41_square.png}
    %\caption{Preference of automatic CL}
    %\end{subfigure}
    \includegraphics[width=0.8\columnwidth]{Figure/Bipedal/fig2_combined.png}
    \caption{{\bf (a)} Boxplot of the log-scaled eigenvalues of sample covariance matrices of the trained embeddings generated by the near optimal policies for different environments. 
    %where we take average over environments with the same height. 
    {\bf (b)} Task preference of automatically generated curriculum at 5M and 10M training steps respectively. The red regions are the regions where a task has a higher probability to be sampled.}
    \label{fig:cov_mat}
\end{figure}
\vspace{-10pt}

==> Submission/math_definitions.tex <==
% \newcommand{\vect}[1]{}
\newcommand{\expl}{\operatorname{expl}}
\newcommand\barbelow[1]{\stackunder[1.2pt]{$#1$}{\rule{.8ex}{.075ex}}}



